GIVEPose: Gradual Intra-class Variation Elimination for RGB-based Category-Level Object Pose Estimation

Recent advances in RGBD-based category-level object pose estimation have been limited by their reliance on precise depth information, restricting their broader applicability. In response, RGB-based methods have been developed. Among these methods, geometry-guided pose regression that originated from instance-level tasks has demonstrated strong performance. However, we argue that the NOCS map is an inadequate intermediate representation for geometry-guided pose regression method, as its many-to-one correspondence with category-level pose introduces redundant instance-specific information, resulting in suboptimal results. This paper identifies the intra-class variation problem inherent in pose regression based solely on the NOCS map and proposes the Intra-class Variation-Free Consensus (IVFC) map, a novel coordinate representation generated from the category-level consensus model. By leveraging the complementary strengths of the NOCS map and the IVFC map, we introduce GIVEPose, a framework that implements Gradual Intra-class Variation Elimination for category-level object pose estimation. Extensive evaluations on both synthetic and real-world datasets demonstrate that GIVEPose significantly outperforms existing state-of-the-art RGB-based approaches, achieving substantial improvements in category-level object pose estimation. Our code is available at https://github.com/ziqin-h/GIVEPose.

==> tab/camera_percat.tex <==
\begin{table*}[b]
    \centering
    \tablestyle{16pt}{1.1}
    \begin{tabular}{@{}l|c c c|c c c c c@{}}
    % \toprule
        Category & $NIoU_{25}$ & $NIoU_{50}$ & $NIoU_{75}$ & $10^\circ 0.2d$ & $10^\circ 0.5d$ & $0.2d$ & $0.5d$ & $10^\circ$ \\ 
        \shline
        bottle & 78.0 & 57.6 & 20.4 & 56.1 & 82.6 & 56.2 & 83.2 & 87.4 \\ 
        bowl   & 95.4 & 86.7 & 35.6 & 82.5 & 95.6 & 82.9 & 96.3 & 95.9 \\
        camera & 60.0 & 23.9 & 3.3 & 18.1 & 59.9 & 21.5 & 72.6 & 72.2 \\ 
        can   & 76.5 & 52.1 & 13.4 & 43.6 & 78.5 & 43.6 & 78.5 & 87.2 \\ 
        laptop & 92.1 & 74.8 & 39.3 & 68.2 & 89.5 & 72.0 & 95.6 & 91.7 \\ 
        mug  & 54.8 & 24.8 & 4.2 & 16.3 & 7.2 & 22.1 & 64.1 & 59.8 \\
        \hline
        average &76.1 & 53.3& 19.4 & 47.5 & 75.5 & 82.4 & 49.7 & 81.7 \\ 
        % \bottomrule
    \end{tabular}    
    \caption{
    \label{tab:camera_percat}
    Per-category results on the CAMERA25 dataset \cite{wang2019normalized} using scale-agnostic evaluation metrics.}    
\end{table*}

==> tab/real_percat.tex <==
\begin{table*}[b]
    \centering
    \tablestyle{16pt}{1.1}
    \begin{tabular}{@{}l|c c c|c c c c c@{}}
    % \toprule
        Category & $NIoU_{25}$ & $NIoU_{50}$ & $NIoU_{75}$ & $10^\circ 0.2d$ & $10^\circ 0.5d$ & $0.2d$ & $0.5d$ & $10^\circ$ \\ 
        \shline
        bottle & 26.6 & 4.6 & 0.5 & 4.6 & 39.6 & 4.8 & 43.5 & 49.7 \\ 
        bowl   & 100.0 & 98.9 & 73.5 & 97.9 & 99.9 & 98.1 & 100.0 & 99.9 \\
        camera & 60.2 & 26.3 & 1.3 & 10.2 & 27.8 & 21.1 & 69.8 & 30.8 \\ 
        can   & 61.3 & 32.8 & 6.1 & 41.7 & 86.7 & 41.9 & 88.7 & 90.4 \\ 
        laptop & 85.4 & 70.2 & 33.2 & 56.6 & 66.6 & 61.8 & 85.4 & 67.2 \\ 
        mug  & 95.1 & 69.3 & 10.2 & 56.7 & 68.5 & 65.8 & 99.2 & 68.5 \\
        \hline
        average &71.4 & 50.3& 20.8 & 44.6 & 64.8 & 48.9 & 81.1 & 67.8 \\
        % \bottomrule
    \end{tabular}    \caption{\label{tab:real_percat}Per-category results on the REAL275 dataset using scale-agnostic evaluation metrics.}    
\end{table*}

==> tab/sup_exp1.tex <==
\begin{center}
\scriptsize
\vspace{-0.8em}
\begin{tabular}{@{}l|c c|c c@{}}
% \toprule
    Method & $NIoU_{50}$ & $NIoU_{75}$ & $10^\circ 0.2d$ & $10^\circ 0.5d$  \\ 
    \shline
    Ours & \textbf{50.3} & \textbf{20.8} & \textbf{44.6} & \textbf{64.8}  \\ 
    \hline
    Ball alone  & 48.3 & 15.6 & 42.4 & 61.8 \\
    N2I2B       & 47.7 & 20.0 & 40.3 & 60.2 \\ 
    w/o concat* & 6.9 (50.8) & 0.1 (14.7) & 0.5 (43.7) & 3.9 (65.9) \\

    % \bottomrule
\end{tabular}
\vspace{-0.8em}
\end{center}


% \begin{wraptable}
%     \centering
%     \tiny
%     \tablestyle{4pt}{1.2}
%     \begin{tabular}{@{}l|c c|c c@{}}
%     % \toprule
%         Method & $NIoU_{50}$ & $NIoU_{75}$ & $10^\circ 0.2d$ & $10^\circ 0.5d$  \\ 
%         \shline
%         Ours & \textbf{50.3} & \textbf{20.8} & \textbf{44.6} & \textbf{64.8}  \\ 
%         \hline
%         Ball alone  & 48.3 & 15.6 & 42.4 & 61.8 \\
%         N2I2B  & 47.7 & 20.0 & 40.3 & 60.2 \\ 
        

%         % \bottomrule
%     \end{tabular}
%     \label{tab:ablation}
% \end{wraptable}

==> tab/sup_exp2.tex <==
\begin{center}
\scriptsize
\vspace{-0.8em}
\begin{tabular}{@{}l|c |c c|c c@{}}
% \toprule
    Method & Coordinate map &$IoU_{25}$ & $IoU_{50}$ & $10^\circ10cm$ & $10cm$  \\ 
    \shline
    Ours & - & 42.9 & \textbf{20.1} & \textbf{34.2} & 45.9  \\ 
    \hline
    PnP  & NOCS (GIVE)  & 41.5 & 19.5 & 33.9 & 45.0 \\
    PnP  & NOCS (only)  & 22.9 & 6.5  & 31.5 & 43.3 \\
    PnP  & IVFC (GIVE)  & \textbf{43.0} & 19.3 & \textbf{34.2} & \textbf{48.6} \\ 
    PnP  & IVFC (only)  & 19.3 & 4.8  & 31.4 & 44.7       
    % \bottomrule
\end{tabular}
\vspace{-0.8em}
\end{center}

==> tab/wild6d_percat.tex <==
\begin{table*}[b]
    \centering
    \tablestyle{16pt}{1.1}
    \begin{tabular}{@{}l|c c c|c c c c c@{}}
    % \toprule
        Category & $NIoU_{25}$ & $NIoU_{50}$ & $NIoU_{75}$ & $10^\circ 0.2d$ & $10^\circ 0.5d$ & $0.2d$ & $0.5d$ & $10^\circ$ \\ 
        \shline
        bottle & 87.3 & 62.4 & 17.4 & 57.1 & 76.7 & 68.9 & 94.9 & 77.3 \\ 
        bowl   & 99.3 & 91.8 & 42.9 & 87 & 96.2 & 88.5 & 99.7 & 96.3 \\
        camera & 60.8 & 22.0 & 0.3 & 1.2 & 2.8 & 26.4 & 73.4 & 3.0 \\ 
        laptop & 99.7 & 99.6 & 79.9 & 18 & 18.1 & 99.4 & 99.7 & 18.1 \\ 
        mug  & 89.6 & 26.4 & 0.1 & 3.9 & 7.5 & 24 & 93.7 & 7.5 \\
        \hline
        average &87.3 & 60.4& 28.1 & 33.4 & 40.3 & 61.4 & 92.3 & 40.4\\
        % \bottomrule
    \end{tabular}    
    \caption{\label{tab:wild_percat}
    Per-category results on the Wild6D dataset \cite{fu2022wild6d} using scale-agnostic evaluation metrics.}    
\end{table*}
